Bidder Selection Problem in Position Auctions: A Fast and Simple Algorithm via Poisson Approximation

In the Bidder Selection Problem (BSP) there is a large pool of $n$ potential advertisers competing for ad slots on the user's web page. Due to strict computational restrictions, the advertising platform can run a proper auction only for a fraction $k<n$ of advertisers. We consider the basic optimization problem underlying BSP: given $n$ independent prior distributions, how to efficiently find a subset of $k$ with the objective of either maximizing expected social welfare or revenue of the platform. We study BSP in the classic multi-winner model of position auctions for welfare and revenue objectives using the optimal (respectively, VCG mechanism, or Myerson's auction) format for the selected set of bidders. Previous PTAS results for BSP optimization were only known for single-item auctions and in case of [Segev and Singla 2021] for $l$-unit auctions. More importantly, all of these PTASes were computational complexity results with impractically large running times, which defeats the purpose of using these algorithms under severe computational constraints. We propose a novel Poisson relaxation of BSP for position auctions that immediately implies that 1) BSP is polynomial-time solvable up to a vanishingly small error as the problem size $k$ grows; 2) there is a PTAS for position auctions after combining our relaxation with the trivial brute force algorithm. Unlike all previous PTASes, we implemented our algorithm and did extensive numerical experiments on practically relevant input sizes. First, our experiments corroborate the previous experimental findings of Mehta et al. that a few simple heuristics used in practice perform surprisingly well in terms of approximation factor. Furthermore, our algorithm outperforms Greedy both in running time and approximation on medium and large-sized instances.

==> lunit.tex <==
In this section, we consider the Bidder Section Problem (BSP) for $\ell$-unit auctions. It serves as a warm-up for more general position auctions presented in \cref{sec:position_auction}. Our main goal here will be to illustrate our approach and analysis ideas rather than to derive independent results for $\ell$-unit auctions. We still obtain an independent result for single-item auction with better approximation guarantees than our more general result for position auctions.

In \cref{sec:math_formulation}, we wrote the expected welfare $\SW(\vars, \l)$ as an integral of $\objb(\bprobs, \l)$. We will introduce several approximations of $\objb$ that make the optimization problem \eqref{eq:lunit_program} easy to solve.

\subsection{Chernoff Approximation}
\label{subsec:lunit_chernoff}

\begin{definition}[Chernoff Objective]
  \label{def:objc}
  For a real vector $\bprobs\in[0,1]^{n}$ and $\ell$, the \textbf{Chernoff objective term} of $\bprobs$ and $\ell$ is a function $\objc(\bprobs,\ell)$:
  \begin{equation*}
    \objc(\bprobs,\ell)
    \eqdef
    \min\left(\Exlong[\vbers\sim\ber(\bprobs)]{\sum_{i=1}^{n}\tmprvi}, \, \ell\right)
    =
    \min\left(\sum_{i=1}^{n}\bprobi, \, \ell\right).
  \end{equation*}
\end{definition}

Formally, we have the following approximation guarantees of $\objb$ by $\objc$:
\begin{restatable}{lemma}{ChernoffObjective}
  \label{lem:chernoff_objective_ratio}
  For all $\bprobs\in[0,1]^n, \ell \in \mathbb N^+$, let $\lambda = \sum_{i=1}^{n}\bprobi$, the following properties hold.
  \begin{flalign*}
    \hspace{1em} & \textup{(a)} & & \objb(\bprobs,\ell)\le \objc(\bprobs,\ell)\le 7 \cdot \objb(\bprobs,\ell).\\
    \hspace{1em} & \textup{(b)} & & \objc(\bprobs,\ell) - \objb(\bprobs,\ell) \le \frac{3}{\sqrt{\lambda}} \cdot \objc(\bprobs, \ell)\le
    \frac{21}{\sqrt{\lambda}} \cdot \objb(\bprobs, \ell). & \\
    \hspace{1em} & \textup{(c)} & & \objc(\bprobs,\ell) - \objb(\bprobs,\ell)
    \le \frac{5}{\sqrt{\ell}} \cdot \objc(\bprobs,\ell)
    \le \frac{35}{\sqrt{\ell}} \cdot \objb(\bprobs,\ell). 
  \end{flalign*}
\end{restatable}

The proof of \cref{lem:chernoff_objective_ratio} is deferred to \cref{subsec:proof_chernoff_objective}. It is a rather straightforward application of Chernoff bounds with careful handling of extreme cases.
The merit of such an approximation is that $\objc$ is a simple concave function which admits efficient maximization algorithms:

\begin{claim}
  \label{cl:chernoff_objective_concavity}
  For all input distributions $\dists$ and $\ell\in\mathbb N^+$, the following properties hold.
  \begin{enumerate}[\hspace{1em}\normalfont(a)]
  \item When $\ell$ is fixed, $\objc(\bprobs,\ell)$ is a concave function of $\bprobs$.
  \item When $\dists$ and $\ell$ are fixed, the approximate social welfare
    \begin{flalign*}
      \hspace{2em} \tilde{\SW}(\vars)\eqdef\int_{0}^{+\infty}\objc(\bprobs(\vars,\tau),\ell) \, \d\tau \quad\text{is a concave function of }\vars. &&
    \end{flalign*}
  \end{enumerate}
\end{claim}
\begin{proof}
  We first prove (a). Let $\lambda=\sum_{i=1}^{n}\bprobi$, then $\objc(\bprobs,\ell)=\min(\lambda,\ell)$ is a concave function of $\lambda$. As $\lambda$ is linear in $\bprobs$, $\objc(\bprobs,\ell)$ is a concave function of $\bprobs$.
  To prove (b), recall that $\bprobi(\vari,\tau)=\vari\cdot\left(1-\disti(\tau)\right)$. Note that $\bprobs(\vars,\tau)$ is linear in $\vars$ for $\forall\tau\in[0,+\infty)$.
  Furthermore, $\objc(\bprobs(\vars,\tau),\ell)$ is a concave function in $\bprobs$ by (a) and thus is concave in $\vars$. Thus $\tilde{\SW}$ is an integral (i.e., linear combination with positive coefficients) of concave functions in $\vars$, which implies that $\tilde{\SW}$ is concave in $\vars$.
\end{proof}

\paragraph{Algorithm for Inputs with Large $\ell$.} 
With \cref{lem:chernoff_objective_ratio} and \cref{cl:chernoff_objective_concavity}, we are ready to present our \cref{alg:large_ell} for the case when $\ell$ is large.

\begin{figure}[ht]
  \begin{tcolorbox}[left=2mm, right=2mm, top=-2mm, bottom=2mm]
    \captionof{algocf}{Approximation to Fractional BSP for $\l$-unit Auctions with Large $\ell$.}{\label{alg:large_ell}}
    Return the optimal solution $\tilde{\vars}^*$ to the continuous concave optimization program in $\vars$:
    \[
      \hspace{-5pt}\begin{array}{lll}
        \text{Maximize} & \SWm(\vars, \ell)
                          = \int_{0}^{+\infty} 
                          \min \left( \sum_{i=1}^{n}\vari\left(1-\disti(\tau)\right), \, \ell \right)
                           \, \d \tau
        \\
        \text{Subject to} & \sum_{i=1}^{n} \vari \le k,
                            \quad \vari \in [0,1], \forall i \in \{1,2,\dots,n\}.
      \end{array}
    \]
  \end{tcolorbox}
\end{figure}

To analyze \cref{alg:large_ell}, first notice that according to \cref{cl:chernoff_objective_concavity}, the optimization program is concave. Thus, we can use standard concave optimization methods like gradient ascent or the ellipsoid method to solve the program in polynomial time\footnote{The function inside the integral is piece-wise constant with finitely many points of discontinuity at  $\tau\in\cup_{i\in[n]}\supp(\disti)$. Thus it can be precisely and efficiently computed in polynomial time.}. Moreover, by \cref{lem:chernoff_objective_ratio} (c), we have for any $\vars\in[0,1]^n$ and $\tau\geq 0$,
\begin{equation*}
  \objc(\bprobs(\vars,\tau),\ell)-\objb(\bprobs(\vars,\tau),\ell)\leq
  \frac{5}{\sqrt{\ell}}\cdot\objc(\bprobs(\vars,\tau),\ell).
\end{equation*}
We get $\tilde{\SW}(\vars)-\SW(\vars)\leq \frac{5}{\sqrt{\ell}}\cdot \tilde{\SW}(\vars)$ by integrating the above bound over $\tau\in[0,\infty)$ for each $\vars\in[0,1]^n$. Similarly, by integrating the bound from \cref{lem:chernoff_objective_ratio} (a) over $\tau\in[0,\infty)$, we get
$\tilde{\SW}(\vars)\geq \SW(\vars)$. 
Now, let $\vars^*$ be the optimal solution to the fractional BSP. Then
\begin{equation*}
  \hspace{-3pt}\SW(\tilde{\vars}^*) \geq \left(1 - \frac{5}{\sqrt{\ell}}\right)\tilde{\SW}(\tilde{\vars}^*)
  \geq \left(1 - \frac{5}{\sqrt{\ell}}\right)
  \tilde{\SW}(\vars^*) 
   \geq \left(1 - \frac{5}{\sqrt{\ell}}\right)
   \SW(\vars^*),
\end{equation*}
where to get the first inequality we use the upper bound on 
$\tilde{\SW}$ for $\vars=\tilde{\vars}^*$; the second inequality 
holds, as $\tilde{\vars}^*$ maximizes the $\tilde{\SW}$ objective; the third inequality is a lower bound on 
$\tilde{\SW}$ for $\vars=\vars^*$.
This means that $\tilde{\vars}^*$ is an $\big( 1 - \frac{5}{\sqrt{\ell}} \big)$-approximate solution.

Thus \cref{alg:large_ell} runs in polynomial time and its approximation ratio gets closer to $1$ as $\ell$ gets larger. I.e., informally speaking, the problem gets easier as $\ell$ grows.

\subsection{Poisson Approximation}
\label{subsec:lunit_poisson}
The previous section~\ref{subsec:lunit_chernoff} covers the case of large $\ell$. The same approach also works for thresholds $\tau$ with large $\sum_i \bprobi(\vari,\tau)$. However, Chernoff bounds are not good for small probability tail events, which typically are the main contributors to the welfare for small $\ell$. To handle these tail events we use \emph{Poisson approximation}, which is the central idea of our paper. 


\begin{definition}[Poisson Objective]
  \label{def:objp}
  For a real vector $\bprobs \in [0, 1]^n$ and integer $\l$, the \textbf{Poisson objective term} is a function $\objp(\bprobs, \l)$ given by
  \[
    \hspace{-3pt}\objp(\bprobs, \l) \eqdef
    \ExlongNobody[\vpoiss \sim \pois(\bprobs)] \Bk{\min\bk{\sum_{i=1}^n \vpoisi, \, \l}}
    =
    \Exlong[\sumpois \sim \pois(\sum_{i=1}^n \bprobi)]{\min\bk{\sumpois, \, \l}}.
  \]
\end{definition}

Note that the latter equality is an important property of Poisson distribution: the sum of independent Poisson random variables $\vpoisi \sim \pois(\bprobi)$ follows the Poisson distribution $\pois(\sum_{i=1}^n \bprob_i)$. Another crucial property is concavity of the Poisson approximation.

\begin{claim}[Concavity of Poisson]
  \label{cl:objp_concave}
  $\objp(\bprobs, \l)$ is a concave function in $\bprobs \in [0,1]^n$ for $\forall\l\in\N$.
\end{claim}

\begin{proof}  
  Let $\lambda = \sum_{i = 1}^n \bprobi$. Notice that $\objp(\bprobs, \l)$ only depends on $\lambda$, which is linear in $\bprobs$. We use $\objp(\lambda)$ to represent this function. Then, we only need to prove that $\objp(\lambda)$ is concave in $\lambda$.
  We first rewrite
  \begin{equation*}
    \objp(\lambda) = \l - \sum_{j = 0}^{\l - 1} \Prlong[\sumpois \sim \Pois(\lambda)]{\sumpois = j} \cdot (\l - j) 
    = \l - \sum_{j = 0}^{\l - 1} \frac{\lambda^{j}}{j!} e^{-\lambda} \cdot (\l - j).
  \end{equation*}
  Then by a straightforward differentiation of the partial series we get
  \begin{equation*}
    \frac{\d}{\d \lambda} \objp = \sum_{j = 0}^{\l - 1} \frac{\lambda^j}{j!} e^{-\lambda}, \quad\quad
    \frac{\d^2}{\d \lambda^2} \objp = -e^{-\lambda} \frac{\lambda^{\l - 1}}{(\l - 1)!} < 0.
  \end{equation*}
  Therefore, $\objp(\bprobs, \l)$ is concave in $\lambda$, and thus concave in $\bprobs$.
\end{proof}

\paragraph{Approximation Guarantees.}

There are many known Poisson approximation results (see, e.g., a survey~\cite{Novak19}) for the sum of independent Bernoulli random variables, e.g., in total variation, earth mover's, uniform (a.k.a.~Kolmogorov) distances. These are typically absolute approximation guarantees, while we need relative approximations similar to Chernoff approximations from \cref{lem:chernoff_objective_ratio}. As our goal is to handle small probability tail events, we assume that each bidder's value $\vali$ has only a small probability $\delta$ to be greater than zero, i.e., $\forall i \in [n], \; \Prx{\vali \! > \! 0} \le \delta$. The following Poisson absolute approximation result will be useful to us:

\begin{restatable}[\textup{\cite[Lemma 11.3.V, p$.$\,162]{daley2008pointprocesses}}]{lemma}{CiteCombined}
  \label{lem:cite_combined}
  Let $(z_i\sim\ber(q_i))_{i=1}^n$ be $n$ independent Bernoulli random variables with $q_i\le\delta$ for $\forall i \in [n]$. Let $Z \eqdef \sum_{i=1}^n z_i$ and $\sumpois \sim \Pois(\lambda)$, where $\lambda \defeq \sum_{i=1}^n \bprob_i$.
  Then 
  \begin{align*}
    \textup{(total variation distance)} \quad
    \sum_{j = 0}^{\infty} \absFix{ \Pr[Z = j] - \Pr[\sumpois = j]} \le \delta.
    \numberthis \label{eq:cite_2}
  \end{align*}
\end{restatable}

With the help of \cref{lem:cite_combined} we can derive relative approximations:

\begin{restatable}{lemma}{PoissonApproximationRatio}
  \label{lem:objp_ratio}
  Suppose $\bprobs \in [0, \delta]^n$ and $\ell\in\N$. Then
  \begin{align*}
    \textup{(a)} &&& \absFix{\objb(\bprobs, \l) - \objp(\bprobs, \l)} \le \LeadingFactorDelta \cdot \delta \cdot \objb(\bprobs, \l) && (\forall \delta, \, \ell), \\
    \textup{(b)} &&& 0 \le \objb(\bprobs, 1) - \objp(\bprobs, 1) \le  \delta \cdot \objb(\bprobs, 1) && (\ell=1).
  \end{align*}
\end{restatable}

The proof of \cref{lem:objp_ratio} is deferred to \cref{subsec:proof_PoissonApproximationRatio}.

\paragraph{Algorithm for Small Tail Probabilities.} Assume that each bidder's value $\vali$ has at most $\delta$ probability to be greater than zero. Then \cref{lem:objp_ratio} and \cref{cl:objp_concave} suggest \cref{alg:low_nonzero}.
\begin{figure}[ht]
  \begin{tcolorbox}[left=2mm, right=2mm, top=-2mm, bottom=2mm]
    \captionof{algocf}{Approximation to Fractional BSP for Tail Probabilities $\l$-unit Auctions.}{\label{alg:low_nonzero}}
    Return the optimal solution $\tilde{\vars}^*$ to the concave program:
    \[
      \begin{array}{lll}
        \text{Maximize} & \SWm(\vars, \ell)  
                          \eqdef\int_{0}^{+\infty} \objp(\bprobs(\vars, \tau), \l) \, \d \tau \\
        \text{Subject To} & \sum_{i=1}^{n} \vari \leq k, 
                            \quad \vari \in [0,1], \forall i \in \{1,2,\dots,n\}.
      \end{array}
    \]
  \end{tcolorbox}
\end{figure}

We can solve the above program efficiently via standard concave function maximization methods, as the objective $\SWm$ is concave in $\vars$.
Indeed, from \cref{cl:objp_concave} we know that $\objp(\bprobs, \l)$ is concave in $\bprobs$ and, since $\bprobs(\vars, \tau)$ is linear in $\vars$ for every fixed $\tau$, $\objp$ is also concave in $\vars$. As $\SWmodi(\vars, \l)$ is an integral (non-negative linear combination) of $\objp(\bprobs(\vars, \tau), \l)$, $\SWm$ is concave in $\vars$.

From \cref{lem:objp_ratio}, we obtain the following approximation guarantees of $\SW(\vars, \ell)$ by  $\SWm(\vars, \l)$.
\begin{align*}
  \absFix{\SW(\vars, \l) - \SWmodi(\vars, \l)}
  &\le \int_{0}^{+\infty} \absFix{\objb(\bprobs(\vars, \tau), \l) - \objp(\bprobs(\vars, \tau), \l)} \,\d \tau\\
  &\le \LeadingFactorDelta \, \delta \cdot \SW(\vars, \l).
    \numberthis \label{eq:swmodi_p_ratio}
\end{align*}
Let $\vars^{*}$ be the best solution of the original problem \eqref{eq:lunit_program}. We have
\begin{align*}
  \SW(\tilde{\vars}^*, \l) &\ge \SWm(\tilde{\vars}^*, \l) - \LeadingFactorDelta \, \delta \,\cdot\, \SW(\tilde{\vars}^*, \l) \\
  &\ge \SWm(\vars^{*}, \l) - {}
  \LeadingFactorDelta \, \delta \,\cdot\, \SW(\vars^{*}, \l) 
  \ge \bk{1 - \TwiceLeadingFactorDelta \, \delta} \SW(\vars^{*}, \l).
\end{align*}
Hence, \cref{alg:low_nonzero} is $\midbk{1 - \TwiceLeadingFactorDelta \, \delta}$-approximation.

\subsection{Single-Item Auction}
\label{subsec:single_item}
We saw in \cref{subsec:lunit_chernoff} that BSP gets easier as $\l$ grows. We also applied a Poisson approximation framework in the previous section \ref{subsec:lunit_poisson} to handle BSP for small probability tail events. Here we illustrate how to apply Poisson approximation to the case of small $\l$ without any assumption on the distributions $\dists$. We focus on the case of $\l=1$, i.e., single-item auction, as it was extensively studied in previous work.

The idea to avoid the extra assumption $\Prx{\vali>0}\le\delta$ is a simple resource augmentation argument: reserve a small fraction $\eps\cdot k$ of bidders, which affects the final approximation by at most $(1-\eps)$ factor due to the submodularity of BSP as a set function of the invited bidders.
We adopt the following variant for our Poisson approximation, which is inspired by the so-called Core-Tail decomposition from \cite{mehta2020hitting}.

Recall that for the single-item auction
\[
\SW(\vars) = \int_{0}^{+\infty} \objb(\bprobs(\vars, \tau), 1) \,\d\tau = \int_{0}^{+\infty} \Prlong[\vals \sim \vars \cdot \dists]{\exists \vali \ge \tau} \,\d\tau.
\]
We fix a small set $\Sfix$ of $\eps\cdot k$ bidders, such that $\Prx[\vals \sim \dists]{\exists i\in\Sfix : \vali\ge\eta} \ge 1-\eps$ for a threshold $\eta$. This allows us to take care of thresholds $\tau$ in a low range $\tau\in[0,\eta]$ by including $\Sfix$ in the solution (i.e., make $\vari=1$ for all $i\in\Sfix$). Naturally, we want to pick bidders with higher probabilities $\Prx{\vali>\eta}$ into $\Sfix$, which means that for the high range thresholds $\tau>\eta$ we get the small probability property for each bidder $i\notin \Sfix$. This allows us to reduce BSP to the case of small probabilities tail events for $\tau>\eta$ and bidders $i\in[n]\setminus\Sfix$, which can be effectively solved by the Poisson approximation. Formally, we can get the following guarantees for $\Sfix$.

\begin{claim}[Small Bidder Set]
  \label{cl:core_tail_single_item}
  Let $\eps \ge \sqrt{\frac{\ln k}{k}}$ be a multiple of $1/k$. We can find in polynomial time a threshold $\eta \ge 0$ and a set $\Sfix \subset [n]$ of size $|\Sfix|=\eps\cdot k$, such that
  \[
    \hspace{-3pt} \textup{(a)} \; \Prlong[\vals \sim \dists]{\exists i \in \Sfix : \vali \ge \eta} \ge 1 - \frac{1}{k};
    \quad \textup{(b)} \;
    \forall i \notin \Sfix, \; \Prlong[\vali \sim \disti]{\vali > \eta} < \eps.
  \]
\end{claim}
\begin{proof}
  Recall that all distributions $\{\disti\}_{i\in[n]}$ have finite support. Thus we can search through all thresholds $\tau$ in polynomial time. There must be two consecutive threshold values $\eta$ and $\eta_{+}\!>\eta$ such that the number of bidders $|\{i: \Prx{\vali\ge\eta}\ge\eps\}|\ge \eps\cdot k$ with large tail probabilities $\Prx{\vali\ge\eta}\ge \eps$ is at least $\eps\cdot k$, but a similar number of bidders $|\{i: \Prx{\vali>\eta}=\Prx{\vali\ge\eta_{+}}\ge\eps\}|< \eps\cdot k$
  for the next threshold value $\eta_{+}$ is strictly less than $\eps\cdot k$. 

  Let us place each bidder $i$ with $\Prx{\vali>\eta}\ge\eps$ into $\Sfix$ and fill the remaining positions in $\Sfix$ up to size $\eps\cdot k$ (so that $|\Sfix|=\eps\cdot k$) with bidders from $\{i: \Prx{\vali\ge\eta}\ge\eps > \Prx{\vali\ge\eta_{+}}\}$. Then, every bidder $i\notin\Sfix$ has $\Prx{\vali>\eta}=\Prx{\vali\ge\eta_{+}}<\eps$ as required by condition (b). On the other hand, $|\Sfix|=\eps\cdot k$ and $\Prx{\vali\ge\eta}\ge\eps$ for every $i\in\Sfix$, i.e., condition (a) is satisfied since 
  \[
    \Prlong[\vals\sim\dists]{\exists i\in\Sfix: \vali\ge\eta} \ge 1-(1-\eps)^{\eps\cdot k}\ge 
    1-e^{-\eps^2\cdot k}\ge 1-\frac{1}{k},
  \]
  where to get the second inequality, we used the fact that $(1-\frac{1}{x})^{x}<e^{-1}$ for any $x\ge 1$.
\end{proof}
After selecting such set $\Sfix$ and threshold $\eta$, we are ready to give the complete description of \cref{alg:single_item}.

\begin{figure}[ht]
  \centering
  \begin{tcolorbox}[left=2mm, right=2mm, top=-2mm, bottom=2mm]
    \captionof{algocf}{Fractional BSP for Single-Item Auction.}{\label{alg:single_item}}
    Fix $\eps = \sqrt{\frac{\ln k}{k}}$ rounded up to a multiple of $1/k$, then do the following steps:
    \begin{enumerate}[(1)]
    \item Find $(\eta, \Sfix)$ as in  \cref{cl:core_tail_single_item}. Set $\vari=1$ for $\forall i\in\Sfix$.
    \item For the remaining bidders $M\eqdef[n]\setminus \Sfix$ let the Poisson approximation $\SWm(\varsM)$ be
      \[
        \qquad \SWm(\varsM) \defeq \bk{1-\frac{1}{k}}\eta + \int_{\eta}^{+\infty} \objpm\bk{\bprobs(\varsM, \tau)} \,\d\tau,
        \numberthis \label{eq:def_swm_single}
      \]
      \begin{align*}
        \text{where} && \objpm\bk{\bprobsM} &\defeq \pbase + \midbk{1 - \pbase} \cdot \objp\bk{\bprobsM, \, \ell=1}, \numberthis \label{eq:def_objpm_single} \\
        \text{and} &&
        \pbase &\defeq \Prlong[\vals \sim \dists]{\exists i \in \Sfix : \vali \ge \tau}.
      \end{align*}
      \item Return $\varsWStar = (\vec{1}_{\Sfix}, \, \varsMWStar)$, where $\varsMWStar$ is the solution to the concave program in $\varsM$:
        \[
          \hspace{-2mm}
          \begin{array}{ll}
            \text{Maximize} & \SWm(\varsM) \\
            \text{Subject To} & \sum_{i \in M} \vari \le k-\eps\cdot k, \quad \vari \in [0,1], \forall i \in M.
          \end{array}
          \hspace{-2mm}
          \numberthis \label{eq:singleitem_program}
        \]
    \end{enumerate}
  \end{tcolorbox}
\end{figure}
In the algorithm, we ignore thresholds $\tau\in[0,\eta]$, as by taking $\Sfix$ we have already achieved high success probability of at least $1-\frac{1}{k}$ by \cref{cl:core_tail_single_item}. For the high range thresholds $\tau>\eta$, we first observe that as the result of fixing set $\Sfix$, the probability that there is a bidder with value greater than the threshold $\tau$ becomes
\[
  \!\!
  \objb(\bprobs,1)=
  \Prx{\exists i\in[n]:\vali\ge\tau}=
  \pbase+\bk{1 - \pbase} \cdot \Prx{\exists i\in M:\vali\ge\tau},
\]
where $\pbase$ is a constant that we can easily compute.
Hence, we respectively adjust the Poisson approximation term $\objpm\midbk{\bprobsM}$ in the algorithm according to \eqref{eq:def_objpm_single} (we slightly abuse notations by writing $\objp\midbk{\bprobsM}$ instead of $\objp\midbk{\bprobs}$: for the coordinates $i\notin M$ we have $\{\bprobi=0, \, i\in\Sfix\}$).

\begin{restatable}{theorem}{thmSingleItem}
  \label{thm:single_item}
  \cref{alg:single_item} for single-item auction works in polynomial time and is a $\midbk{1 - 2\eps}$-approximation, i.e., a $\bigbk{1 - O\big(\sqrt{\ln k / k}\big)}$-approximation to the fractional BSP.
\end{restatable}
\begin{proof} We first verify that \cref{alg:single_item} is polynomial. Note that the step (1) works in polynomial time by 
  \cref{cl:core_tail_single_item}. For each $\tau$ in the support of $\disti$ we calculate in polynomial time the constants $\pbase\in[0,1]$. Both $\objpm\midbk{\bprobsM}$ for each $\varsM$ and $\tau$ in the support and $\SWm(\varsM)$ for each $\varsM$ can be computed in polynomial time. 
  Moreover, all first and second order partial derivatives of $\SWm(\varsM)$ can be computed in the same way as the integral of respective derivatives of $\objpm\midbk{\varsM}$. Furthermore, it is easy to see that $\SWm(\varsM)$ is a concave function in $\varsM$, since it is a positive linear combination of constant terms (such as $(1-1/k)\eta$ and $\pbase$) and concave functions $\objp\midbk{\varsM}$ according to \cref{cl:objp_concave}. Hence, we can find the optimal solution $\conpx$ in polynomial time using standard concave (first or second order) maximization methods.

  To prove an approximation guarantee of $1-2\eps$ for \cref{alg:single_item}, we first derive the following approximations of $\SW(\varsM,\onevec_{\Sfix})$ by $\SWm(\varsM)$ similar to \eqref{eq:swmodi_p_ratio} (but in a special case of $\l=1$).

  \begin{lemma}
    \label{lem:sw_poisson_single_item}
    $
    \forall\varsM\in[0,1]^{|M|}$, $
    0\le \SW(\varsM,\onevec_{\Sfix}) - \SWm(\varsM) 
    \le \eps \cdot \SW(\varsM,\onevec_{\Sfix}).
    $
  \end{lemma}
  \begin{proof}
    Recall that by \eqref{eq:sw_to_objb} the Social Welfare $\SW(\vars)$ for $\vars=(\varsM,\onevec_{\Sfix})$ and $\ell=1$ is
    \[
      \SW(\vars)=\int_{0}^{\eta}
      \objb(\bprobs(\vars,\tau)) \, \d\tau
      +
      \int_{\eta}^{+\infty} \objb(\bprobs(\vars,\tau)) \, \d\tau.
    \]
    For the low range $\tau\in[0,\eta]$ we have $\objb(\bprobs(\vars,\tau)) \in [1 - \frac{1}{k},\, 1]$ due to the choice of $\Sfix$ in \cref{cl:core_tail_single_item}. It is well approximated by the respective term $\bk{1-\frac{1}{k}}\eta$ in \eqref{eq:def_swm_single}.

    For the high range $\tau>\eta$, we apply \cref{lem:objp_ratio} (b) with $\delta = \eps$ and get the following bound:
    \begin{align*}
      \objb(\bprobs) - \objpm(\bprobs)
      ={}& \midbk{1 - \pbase} \bk{\objb\midbk{\bprobsM} - \objp\midbk{\bprobsM}} \\
      \le{}& \midbk{1 - \pbase}  \eps \cdot \objb\midbk{\bprobsM}
      \le \eps \cdot \objb(\bprobs).
    \end{align*}
    On the other hand, $\objb(\bprobs) - \objpm(\bprobs)\ge 0$, as $\objb(\bprobsM) \ge \objp(\bprobsM)$ by \cref{lem:objp_ratio} (b). Thus
    \begin{align*}
      0\le \SW(\vars) - \SWm(\varsM) &\le 
      \frac{\eta}{k}+ \eps \cdot \int_{\eta}^{+\infty} \objb(\bprobs(\vars, \tau)) \,\d\tau \\
      &\le \max\bk{\frac{1}{k-1},\eps}\SW(\vars)= \eps\cdot\SW(\vars),
    \end{align*}
    where the last equality holds since $\eps\ge\sqrt{\frac{\ln k}{k}}$.
  \end{proof}
  Now we are ready to complete the proof of \cref{thm:single_item}. Let $\optx$ be the optimal solution to fractional BSP. We consider $\optplusfix\in\R^n_{\ge 0}$ defined as $\optplusfix\eqdef(\optpx, \onevec_{\Sfix})$, so that $\optplusfix \succeq \optx$. Then, by \cref{lem:sw_poisson_single_item} for $\vars=\optplusfix$ we have 
  \[
    \SWm(\optpx)\ge(1-\eps)\cdot\SW(\optplusfix)\ge
    (1-\eps)\cdot\SW(\optx).
  \]
  On the other hand, by \cref{lem:sw_poisson_single_item} for $\vars = \conx$ we have
  \begin{align*}
    \SW(\conx)\ge\SWm(\conpx)&\ge\SWm\bk{\frac{k-\eps\cdot k}{k}\cdot\optpx} \\
    &\ge (1-\eps)\cdot\SWm(\optpx)\ge(1-2\eps)\cdot\SW(\optx),
  \end{align*}
  where the second inequality holds, as $\conpx$ is the optimal solution to \eqref{eq:singleitem_program} and $\frac{k-\eps\cdot k}{k}\cdot\varsMStar$ is a feasible solution; the third inequality holds, as $\SWm(\vars)$ is a concave function in $\vars$ by \cref{cl:objp_concave}; the last inequality holds, as 
  $\SWm(\varsMStar) \ge (1-\eps)\cdot\SW(\optx)$ and $(1-\eps)^2\ge 1-2\eps$. This concludes the proof.
\end{proof}


==> position_app.tex <==
\subsection{Proof of Claim~\ref{cl:simple_chernoff}}
\label{subsec:proof_simple_chernoff}

\simplechernoff*

\begin{proofof}{\cref{cl:simple_chernoff}}
  By Chernoff bound, we have
  \begin{equation*}
    \sum_{i=1}^{n-k}\Prlong[\varss\sim\Ber(\varsf)]{|\varss|\geq k+i}\leq \sum_{i=1}^{n-k}e^{-\frac{i^2}{i+2k}}\leq \sum_{i=1}^{\infty}e^{-\frac{i^2}{i+2k}}\le 
    \int_{0}^{\infty}e^{-\frac{x^2}{x+2k}}\,\d x.
  \end{equation*}

We further estimate this integral as 
\begin{equation*}
\int_{0}^{\infty}e^{-\frac{x^2}{x+2k}}\,\d x\le
\int_{0}^{\sqrt{k}}e^{-\frac{x^2}{x+2k}}\,\d x+
\int_{\sqrt{k}}^{\infty}e^{-\frac{x}{1+2\sqrt{k}}}\,\d x \le 1\cdot \sqrt{k} -(1+2\sqrt{k})\left .e^{-\frac{x}{1+2\sqrt{k}}} \right |_{\sqrt{k}}^{+\infty}=O(\sqrt{k}).
\end{equation*}
  
  This concludes the proof of \cref{cl:simple_chernoff}.
\end{proofof}




==> rounding.tex <==
We conclude Section~\ref{sec:position_auction} by presenting the rounding algorithm, which takes our solution $\tilde{\vars}^*$ to the fractional BSP produced by \cref{alg:main} and returns a solution to the integral BSP. 
Recall that the social welfare $\SW(S)$ of a $\l$-unit or position auction is submodular as a function of the invited set of bidders $S$.
\begin{claim}
\label{cl:submodularity}
The expected social welfare $\SW(S)$ for a set of bidders $S\subseteq[n]$ in any $\l$-unit or position auction is a submodular function of $S$.
\end{claim}

Our fractional relaxation works as the standard multi-linear extension of submodular functions, which corresponds to sampling a random set of bidders $S\sim\prod_{i=1}^{n}\Ber(\vari)$ in the integral BSP. To align the notations for fractional and integral BSPs, we shall use vectors $\varss,\varsi\in\{0,1\}^n$ for the respective sets of selected bidders.
Specifically, we use $\varss\sim\Ber(\vars)$ to represent the random set $S$ in the multi-linear extension. Our rounding procedure is quite standard and proceeds as follows.

\begin{figure}[htbp]
  \centering
  \begin{tcolorbox}[left=2mm, right=2mm, top=-2mm, bottom=2mm]
    \captionof{algocf}{Rounding: algorithm for Integral BSP}{\label{alg:int}}
    \begin{enumerate}
    \item Run \cref{alg:main} to obtain a fractional solution $\varsf$.
    \item Sample an integral solution $\varss\sim\Ber(\varsf)$, with $\varss\in\{0,1\}^{n}$.
    \item 
        \begin{itemize}
            \item If $|\varss|_1\le k$, return $\varsi=\varss$, 
            \item Else ($|\varss|_1>k$), return $k$ bidders $\varsi\sim\binom{\varss}{k}$ chosen uniformly at random from $\varss$.
        \end{itemize}
    \end{enumerate}
  \end{tcolorbox}
\end{figure}

\paragraph{Analysis of Algorithm \ref{alg:int}} Clearly, $\varsi$ is a feasible solution to the integral BSP. We will prove below that \cref{alg:int} has almost the same approximation guarantee as \cref{alg:main}. Let us denote the optimal social welfare for integral BSP as $\opt$. Then the best solution $\optx$ to the fractional BSP~ \eqref{eq:pos_original_program} may have only higher welfare $\SW(\optx,\weights)\ge\opt$. Furthermore, since \eqref{eq:pos_original_program} is a multi-linear extension of the integral BSP, we have 
\[
  \Exlong[\varss\sim\Ber(\varsf)]{\SW(\varss,\weights)}=\SW(\varsf,\weights)\ge\bk{1 - \TwiceMaxFactorPlusOne \, k^{-1/4}} \SW(\optx,\weights)
  \ge\bk{1 - \TwiceMaxFactorPlusOne \, k^{-1/4}} \opt.
\]
Our solution $\varsi$ suffers an additional loss when the sample vector $\varss$ has more than $k$ elements $|\varss|_1>k$. On the other hand, for each given $\varss$ with $|\varss|_1>k$ we have $\Ex[\varsi\sim\binom{\varss}{k}]{\SW(\varsi,\weights)}\ge\frac{k}{|\varss|_1}\SW(\varss,\weights)$, due to submodularity of $\SW(\varss,\weights)$ (here we use a standard fact about monotone non-negative submodular function $f$: a uniformly sampled subset $T\subset S$ of given size $|T|=k$ has $\Ex[T]{f(T)}\ge\frac{k}{|S|}f(S)$). Thus 
\begin{align*}
  \Exlong[\varss\sim\Ber(\varsf)]{\SW(\varss,\weights)-\SW(\varsi,\weights)} \le \Exlong[\varss\sim\Ber(\varsf)]{\ind{|\varss|_1>k}\cdot \frac{|\varss|_1-k}{|\varss|_1} \cdot \SW(\varss,\weights)}.
\end{align*}
Furthermore, as $\opt=\max_{S\subseteq[n]:|S|=k}\SW(S,\weights)$ we have $\opt \ge \Ex[\varsi\sim\binom{\varss}{k}]{\SW(\varsi,\weights)} \ge \frac{k}{|\varss|_1}\SW(\varss,\weights)$ for each $\varss$ with $|\varss|_1>k$.
Therefore,
\begin{multline*}
  \Exlong[\substack{\varss\sim\Ber(\varsf) \\ \varsi \sim \binom{\varss}{k}}]{\SW(\varss,\weights)-\SW(\varsi,\weights)} \le \Exlong[\varss\sim\Ber(\varsf)]{\ind{|\varss|_1>k}\cdot \frac{|\varss|_1-k}{k} \cdot \opt}\\
  =\frac{\opt}{k}\cdot\sum_{i=1}^{n-k} i\cdot\Prlong[\varss\sim\Ber(\varsf)]{|\varss|_1=k+i}
  =\frac{\opt}{k}\cdot\sum_{i=1}^{n-k}\Prlong[\varss\sim\Ber(\varsf)]{|\varss|_1\ge k+i}.
\end{multline*}


\begin{restatable}{claim}{simplechernoff}
  \label{cl:simple_chernoff}
  Let $\varsf\in[0,1]^n$ with $|\varsf|_1=k$. Then
$\sum_{i \ge 1}\Prx[\varss\sim\Ber(\varsf)]{|\varss|\geq k+i}=O \bigbk{\sqrt{k}}.$
\end{restatable}

The proof of \cref{cl:simple_chernoff} is a simple application of Chernoff bounds, which we defer to \cref{subsec:proof_simple_chernoff}. \cref{cl:simple_chernoff} allows us to conclude that
$
  \Ex[\varss\sim\Ber(\varsf)]{\SW(\varss,\weights)-\SW(\varsi,\weights)} = O\bigbk{\frac{1}{\sqrt{k}}}\cdot \opt
$, i.e.,
\begin{align*}
  \Exlong[\varss\sim\Ber(\varsf)]{\SW(\varsi,\weights)}=\SW(\varsf,\weights) - O\!\left(\frac{1}{\sqrt{k}}\right)\cdot \opt = \bk{1 - \TwiceMaxFactorPlusOne \, k^{-1/4} - O(k^{-1/2})} \opt.
\end{align*}
The following theorem summarizes the above discussion. 
\begin{theorem}
  \label{thm:final}
  \cref{alg:int} works in polynomial time and in expectation is a 
  $\bk{1 - \TwiceMaxFactorPlusOne \, k^{-1/4} - O(k^{-1/2})}$-approximation to the integral BSP for any position auction.
\end{theorem}
Moreover, since $\SW(\varsi)\leq\opt$, by running rounding algorithm a few times and taking the best produced solution, we can get a slightly worse approximation guarantee of
$(1 - O(k^{-1/4})) \opt$
with high probability.

